Do Gradient Inversion Attacks Make Federated Learning Unsafe?

Federated learning (FL) allows the collaborative training of AI models without needing to share raw data. This capability makes it especially interesting for healthcare applications where patient and data privacy is of utmost concern. However, recent works on the inversion of deep neural networks from model gradients raised concerns about the security of FL in preventing the leakage of training data. In this work, we show that these attacks presented in the literature are impractical in FL use-cases where the clients' training involves updating the Batch Normalization (BN) statistics and provide a new baseline attack that works for such scenarios. Furthermore, we present new ways to measure and visualize potential data leakage in FL. Our work is a step towards establishing reproducible methods of measuring data leakage in FL and could help determine the optimal tradeoffs between privacy-preserving techniques, such as differential privacy, and model accuracy based on quantifiable metrics. Code is available at https://nvidia.github.io/NVFlare/research/quantifying-data-leakage.

==> __old_fig3.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% See this for new line in caption: https://tex.stackexchange.com/questions/101595/how-to-add-line-break-to-caption-without-using-caption-package
\begin{figure*}[htbp]
\newcommand{\figwidth}{.16\textwidth}
\newcommand{\figheight}{.95\textwidth}
\centering
\begin{subfigure}{\figwidth}
  \centering
  \includegraphics[height=\figheight]{figs/attack_success_original.png}
  \caption{\scriptsize \\ \centering Original}
  \label{fig:attack_success_a}
\end{subfigure}
\begin{subfigure}{\figwidth}
  \centering
  \includegraphics[height=\figheight]{figs/attack_success_prior_img.png}
  \caption{\scriptsize \\ \centering Prior}
  \label{fig:attack_success_prior_img}
\end{subfigure}
\begin{subfigure}{\figwidth}
  \centering
  \includegraphics[height=\figheight]{figs/attack_success_geiping.png}
  \caption{\scriptsize\centering  w/o BN loss,\hspace{\textwidth} w global ckpt \cite{geiping2020inverting}}
  \label{fig:attack_success_b}
\end{subfigure}
\begin{subfigure}{\figwidth}
  \centering
  \includegraphics[height=\figheight]{figs/attack_success_nockpt.png}
  \caption{\centering\scriptsize w BN loss,\hspace{\textwidth} w/o global ckpt}
  \label{fig:attack_success_c}
\end{subfigure}
\begin{subfigure}{\figwidth}
  \centering
  \includegraphics[height=\figheight]{figs/attack_success_noprior.png}
  \caption{\centering\scriptsize w BN loss,\hspace{\textwidth} w global ckpt (no prior)}
  \label{fig:attack_success_d}
\end{subfigure}
\begin{subfigure}{\figwidth}
  \centering
  \includegraphics[height=\figheight]{figs/attack_success_bnloss.png}
  \caption{\centering\scriptsize \textbf{Ours}: w BN loss,\hspace{\textwidth} w global ckpt (prior)}
  \label{fig:attack_success_noprior}
\end{subfigure}
    \caption{\textbf{Success factors of the inversion attack.} Here, the ``high-risk'' client 9 sends updates based on one iteration and one image in round 10 of an FL experiment. The original training image is shown for comparison (a). The prior image used to initialize the attack is shown in (b). The inversion technique by Geiping et al.~\cite{geiping2020inverting} does not estimate updated BN statistics during training and therefore cannot handle clients with updated BN layers in their architectures (c). The attack also fails if not initialized with the current global model state/checkpoint (ckpt) (d). Both the current global checkpoint and proper accounting for updated BN statistics during training are necessary for the attack to succeed (e) and further improves when using the image prior (f). The patient’s name and date of birth in the original image are randomly generated to illustrate the difficulty of inverting detailed textual information by the gradient inversion attack. \label{fig:attack_success}}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> extra_info.tex <==
\subsection{Additional Information}
\subsubsection{Ethical approval}
No ethical approval was needed for this research as only publicly available data was used.
%
\subsubsection{Data availability}
The data used for training, validation, and testing data is available at: https://www.kaggle.com/tawsifurrahman/covid19-radiography-database
%
\subsubsection{Code availability}
The Clara Train SDK 4.0 is used for local model training and evaluation: https://ngc.nvidia.com/catalog/containers/nvidia:clara-train-sdk
NVIDIA FLARE is used to record model updates in a simulated FL setting: https://nvidia.github.io/NVFlare
The inversion software will be made available upon acceptance.
%
\subsubsection{Competing Interests}
All authors are employees of NVIDIA Corporation. The authors declare that there are no other competing interests.
%
\subsubsection{Author Contribution}
A.H., H.Y., P.M., D.X., and H.R. conceptualized and designed the study. A.H., H.Y., P.M., and H.R. developed the algorithm. A.H. and H.R. lead the experimentation, analysis, and article writing. A.M., W.L., P.D. A.F., M.G.F., J.K., D.X. contributed to interpretation of the data and writing the article.

